Managing Variability in Relational Databases by VDBMS

Variability inherently exists in databases in various contexts which creates database variants. For example, variants of a database could have different schemas/content (database evolution problem), variants of a database could root from different sources (data integration problem), variants of a database could be deployed differently for specific application domain (deploying a database for different configurations of a software system), etc. Unfortunately, while there are specific solutions to each of the problems arising in these contexts, there is no general solution that accounts for variability in databases and addresses managing variability within a database. In this paper, we formally define variational databases (VDBs) and statically-typed variational relational algebra (VRA) to query VDBs---both database and queries explicitly account for variation. We also design and implement variational database management system (VDBMS) to run variational queries over a VDB effectively and efficiently. To assess this, we generate two VDBs from real-world databases in the context of software development and database evolution with a set of experimental queries for each.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> formulas/vCondTypingRules.tex <==

\begin{figure}[H]
%\textbf{V-conditions static semantics: (b: boolean tag, A: plain attribute, k: constant value)}
  \begin{mathpar}
  \small    

  \inferrule[\conjC]
  	{\envCond \vCond_1\\
    	\envCond \vCond_2}
    {\envCond{\vCond_1 \wedge \vCond_2}}
    
  \inferrule[\disjC]
  	{\envCond \vCond_1\\
    	\envCond \vCond_2}
    {\envCond{\vCond_1 \vee \vCond_2}}
    


  \inferrule[\choiceC]
%  	{\defType{\relInContext{\vContext''}}\in \vSch \\
    	{\envCond[\vctx \wedge \dimMeta, \vType]{\vCond_1} \\
        \envCond[\vctx \wedge \neg \dimMeta, \vType]{\vCond_2}}
    {\envCond{\chc[\dimMeta]{\vCond_1, \vCond_2}}}
    

  \inferrule[\notC]
  	{\envCond \vCond}
    {\envCond \neg \vCond}
        
%  \inferrule[]
%  	{\envCond[\vContext \wedge \dimMeta]{\vCond_1} \\
%    	\envCond[\vContext \wedge \neg\dimMeta]{\vCond_2}}
%    {\envCond{\chc{\vCond_1, \vCond_2}}}
    

    
  \inferrule[\attValC]
  	{
	%\defType{\relInContext{\vContext'}}\in \vSch \\
    	\optAtt [ \dimMeta] \in \vType \\
	\taut{\vctx \imply { \dimMeta}} \\
        \cte \in \dom \vAtt}
    {\envCond{\op \pAtt \cte}}
    
  \inferrule[\boolC]
  	{}
    {\envCond \bTag}
    

    
  \inferrule[\attAttC]
  	{
	%\defType{\relInContext{\vContext'}}\in \vSch \\
    	\optAtt [\dimMeta_1] [\vAtt_1]\in \vType \\
         {\optAtt [\dimMeta_2] [\vAtt_2]} \in \vType \\
         \taut{\vctx \imply \dimMeta_1} \\
         \taut{\vctx \imply \dimMeta_2} \\
        \type[\vAtt_1] = \type[ \vAtt_2]}
    {\envCond{\op{\pAtt_1}{\pAtt_2}}}
    
  \end{mathpar}

\caption{V-condition typing relation. A v-condition \vCond\ is well-typed if 
it is valid in the variational context \vctx\ and type environment \vType, i.e., 
\envCond \vCond. Note that the type rules for v-conditions return a boolean, if
the v-condition is type-correct the rules return \t, otherwise they return \f.}
\label{fig:v-cond-rules}
\end{figure}
%
%\rewrite{reorder this if space allowed!!}


==> sections/SqlGenEx.tex <==
\section{Generated SQL Query}
\label{app:sqlGen.tex}

%\tbf



==> sections/confVQ.tex <==
\subsubsection{Configure V-Query}
\label{sec:conf-vq}

A v-query simply packs multiple relational queries over variants of a VDB
into a single query. As shown in \figref{arch}, after type checking a query,
one of the approaches of 
evaluating a v-query requires configuring the v-query for all possible valid 
configurations which is provided by the feature model of the VDB). 
\figref{v-alg-conf-sem} defines the configuration semantics of VRA which
uses a translator of non-variational queries of VRA to relational algebra. 
As a reminder, both relational
algebra and VRA are domain-specific languages (DSLs) with their own
\eric{could you say this in simpler manner? do we need to provide def 
of trans?}
data types. Hence, configuring
a v-query requires representing the non-variational parts of the v-query in 
relational algebra, done by the translator.
\exref{conf-vq} illustrate configuring a v-query.


\begin{example}
\label{eg:conf-vq}
\tbf
%Assume we have the \vqTxt\ $\vQ_2$ given in Example~\ref{eg:points-for-presence-cond-v-q}.
%We want to get the plain query of $\vQ_2$ associated to the configuration $\config = \left(\US \wedge \neg \Iceland \wedge \neg \Iran\right) \wedge \left(\bank \wedge\neg \invest \wedge\neg \stock\right)$.
%We will have:
%\begin{equation*}
%\eeSem {\vQ_2} = \pi_{\mN} \left(\vRelConfed [\config][\employee]\right)
%\end{equation*}
\end{example}


%\rewrite{sem from old version!}
\input{formulas/vRelAlgConfSem}


==> sections/groupVqProof.tex <==
\section{V-Query Grouping Correctness}
\label{app:vq-group-proof}
%\tbf
%sketch proof or argue why this is true

==> sections/sanityChecks.tex <==

\TODO{double check the following ph and write the properties based on it:}
Conceptually, a variational query describes a query that can
be executed over any database instance consistent with the 
variational schema. The property that must hold between a 
variational query \vQ\ and a variational schema \vSch
is that for every plain query $\pQ_\config$ obtained from \vQ 
by configuring with a function $\config: \fSet \to \bSet$, $\pQ_\config$ 
is consistent with the corresponding plain schema $\pSch_\config$ 
obtained by $\osSem  \vSch$ with the same function \config. That 
is, every variant query matches the corresponding variant schema.
%\REMEMBER{In \secref{prop-q-lang}, we prove that our query language,
%variational relational algebra, can encode this idea and also
%recover any of the conceptually potential results for any instance
%of the variational database.}



==> sections/typeSysPropProof.tex <==
\section{VRA Typing Is Variation Preserving}
\label{app:type-sys-prop-proof}
%\tbf
%vq -c-> q -ts-> T <-c- VT <-ts- vq
%\wrrite{a sen: holds for grouping too!}
%vq -g-> [q] -ts-> [T] == <-g- VT <-ts- vq

==> sections/vsetProps.tex <==
\section{Variational Set Properties}
\label{app:vlist-vset-props}

Variational set as introduced in \secref{vlist-vset} have the following 
properties:
\eric{should I name them?}

$\setDef {\annot [\dimMeta_1 \wedge \dimMeta] {\elem_1},\ldots, \annot [\dimMeta_n \wedge \dimMeta] {\elem_n}}
\equiv 
\setDef {\annot [\dimMeta_1] {\elem_1} ,\ldots, \annot [\dimMeta_n] {\elem_n}}^\dimMeta
$

$ \textit{if } \dimMeta \imply \dimMeta_i \textit{ then: }
\setDef {\annot [\dimMeta_1] {\elem_1},\ldots, \annot [\dimMeta_i] {\elem_i},\ldots, \annot [\dimMeta_n] {\elem_n}}^\dimMeta
\equiv
\setDef {\annot [\dimMeta_1] {\elem_1},\ldots, \annot [\t] {\elem_i},\ldots,\annot [\dimMeta_n] {\elem_n}}^\dimMeta
$

%$\left(e_1^{F_1 \wedge F},\ldots,e_n^{F_n \wedge F}\right)
%\equiv 
%\left(e_1^{F_1},\ldots,e_n^{F_n}\right)^F
%$
%
%$ \textit{if } F \imply F_i \textit{ then: }
%\left(e_1^{F_1},\ldots, e_i^{F_i},\ldots,e_n^{F_n}\right)^F
%\equiv
%\left(e_1^{F_1},\ldots, e_i^\t,\ldots,e_n^{F_n}\right)^F
%$

\moredet{add more properties if needed and space allowed!}

==> sections/writingAdvice.tex <==
Comments by Kent Beck
I will not talk about a topic area, like my distinguished fellow panelists. I will present the process I use as I am writing my papers. You can adapt it for your writing process, or you can use it as a check list for evaluating finished papers (if this is starting to sound like patterns, well, fancy that). Much of what I will say is "common sense," found in any book about writing. Having looked at hundreds of submissions, though, I can state with certainty that most of the authors don't follow this advice.
Write to the program committee. Never forget that before you can write to the vast, eager, and appreciative OOPSLA audience you must first get past the program committee. Before I begin I fix in my mind a picture of a harried PC member, desk piled with papers. Mine comes to the top. I have maybe thirty seconds to grab their interest. Remember that the program committee is made up of experts in the field. Even if your topic is of broad interest to beginners, there must still be some spark in it to keep an expert reading to the end. If your topic is highly technical, it may not be in an area that they are familiar with, so it must readably present the novel aspects of the work.
One startling sentence. Now that you know you are writing to the program committee, you need to find the one thing you want to say that will catch their interest. If you have been working on the world's niftiest program night and day for five years, the temptation is to include absolutely everything about it, "The Foo System In All Its Glory." It'll never work. I know it's painful to ignore all those great insights, but find the most interesting thing you have done and write it down, "network garbage collection is fast and easy." You want the reader's eyes to open wide when they realize what it is you've just said. I think some people are reluctant to boil their message down to one startling sentence because it opens them up to concrete criticism. If you write about the Foo System and someone says it isn't neat, you can just reply, "Is so, nyah!" If you say network garbage collection is easy, it is a statement that is objectively true or false. You can be proven wrong. Wait! You spent five years proving it was easy. Make your case.
Argument: problem, solution, defence, related work. Now that you have a startling sentence, your paper must stand as the argument for its validity. You are convincing the by-now-intrigued committee member of the truth of your amazing statement. Divide your paper into four sections. The first describes the problem to be solved. When the PC member is done reading it, they should understand why it is a problem, and believe that it is important to solve. The second section describes your problem. You are convincing the PC member that your solution really could solve the problem. This section is sometimes supplemented with a section between the defence and related work which describes implementation details. The third section is your defence of why your solution really solves the problem. The PC member reading it should be convinced that the problem is actually solved, and that you have thought of all reasonable counter arguments. The final section describes what other people have done in the area. Upon reading this section, the PC member should be convinced that what you have done is novel.
Abstract. The abstract is your four sentence summary of the conclusions of your paper. Its primary purpose is to get your paper into the A pile. Most PC members sort their papers in an A pile and a B pile by reading the abstracts. The A pile papers get smiling interest, the B pile papers are a chore to be slogged through. By keeping your abstract short and clear, you greatly enhance your chances of being in the A pile. I try to have four sentences in my abstract. The first states the problem. The second states why the problem is a problem. The third is my startling sentence. The fourth states the implication of my startling sentence. An abstract for this paper done in this style would be:
The rejection rate for OOPSLA papers in near 90%. Most papers are rejected not because of a lack of good ideas, but because they are poorly structured. Following four simple steps in writing a paper will dramatically increase your chances of acceptance. If everyone followed these steps, the amount of communication in the object community would increase, improving the rate of progress.
Well, I'm not sure that's a great abstract, but you get the idea. I always feel funny writing an abstract this way. The idea I thought was so wonderful when I started writing the paper looks naked and alone sitting there with no support. I resist the temptation to argue for my conclusion in the abstract. I think it gives the reader more incentive to carefully read the rest of the paper. They want to find you how in the world you could possible say such an outrageous thing. There are my four steps to better papers. You can use them sequentially to write papers, or you can use them to evaluate papers you have already written.
